Creek: Low-latency, Mixed-Consistency Transactional Replication Scheme

In this paper we introduce Creek, a low-latency, eventually consistent replication scheme that also enables execution of strongly consistent operations (akin to ACID transactions). Operations can have arbitrary complex (but deterministic) semantics. Similarly to state machine replication (SMR), Creek totally-orders all operations, but does so using two different broadcast mechanisms: a timestamp-based one and our novel conditional atomic broadcast (CAB). The former is used to establish a tentative order of all operations for speculative execution, and it can tolerate network partitions. On the other hand, CAB is only used to ensure linearizable execution of the strongly consistent operations, whenever distributed consensus can be solved. The execution of strongly consistent operations also stabilizes the execution order of the causally related weakly consistent operations. Creek uses multiversion concurrency control to efficiently handle operations' rollbacks and reexecutions resulting from the mismatch between the tentative and the final execution orders. In the TPC-C benchmark, Creek offers up to 2.5 times lower latency in returning client responses compared to the state-of-the-art speculative SMR scheme, while maintaining high accuracy of the speculative execution (92-100%).

==> algorithms/cabcast_alg.tex <==
\begin{algorithm*}%[p] 
\caption{Conditional Atomic Broadcast for process $p_i$}
\label{alg:cabcast}  
% \algsetup{linenosize=\tiny}
  \normalsize
% \vspace{-0.15cm}
% \begin{multicols*}{2}
\begin{algorithmic}[1]
\State{$\received = \emptyset$ \LineComment{set of messages received by the process}} 
\State{$\unordered = \emptyset$ \LineComment{set of identifiers of messages received but not yet ordered by the process}}
\Statex{\LineComment{each message $\msg$ has a unique identifier denoted by $\id(\msg)$}}
\State{$\ordered = []$ \LineComment{sequence of identifiers of messages ordered but not yet $\cabdeliver$ed by the process}}
\State{$k = 0$ \LineComment{serial number for consensus executions}}

\Procedure{$\cabcast$}{$m : \Message$, $q : \Predicate$}\LineComment{to $\cabcast$ a message $m$ with a test predicate $q : \Message \rightarrow \mathrm{Boolean}$}
  \State{$\msg.m = m$}
  \State{$\msg.q = q$}
  \State{$\rbcast(\msg)$} \label{alg:cabcast:rbcast}
\EndProcedure
  
\Function{$\test$}{$\ids : \sett\langle \Message\ \id\rangle$}
  \State{\Return $\forall \id \in \ids : \exists \msg \in \received : \id(\msg) = \id \wedge \msg.q(\msg.m)$} \label{alg:cabcast:predicate}
\EndFunction
  
\Upon{$\rbdeliver$}{$\msg : \Message$}
  \State{$\received = \received \cup \{ \msg \}$} \label{alg:cabcast:rbdeliver}
  \If{$\id(\msg) \not\in \ordered$}
    \State{$\unordered = \unordered \cup \{ \id(\msg) \}$} \label{alg:cabcast:unordered_add}
  \EndIf
\EndUpon  

\Upon{$\unordered \neq \emptyset$}{} \LineComment{a consensus is run whenever there are unordered messages}
  \State{$k = k + 1$}
  \State{$\propose(k, \unordered, test)$} \LineComment{$k$ distinguishes independent consensus executions} \label{alg:cabcast:propose}
  \State{\textbf{wait until} $\decide(k, \idSet_k)$} \label{alg:cabcast:decide}
  \State{$\unordered = \unordered \setminus \idSet_k$}
  \State{$\idSeq_k = $ elements of $\idSet_k$ (in some deterministic order)} \label{alg:cabcast:order}
  \State{$\ordered = \ordered \cdot \idSeq_k$}
\EndUpon
  
\Upon{$\ordered \neq \emptyset \wedge \exists \msg \in \received : \ordered.\head = \id(\msg) \wedge \msg.q(\msg.m)$}{}
\LineComment{delivers messages ordered and received} \label{alg:cabcast:cabdeliver}
  \State{$\cabdeliver(\msg.m)$} 
  \State{$\ordered = \ordered.\tail$}
\EndUpon
  
\end{algorithmic}
\end{algorithm*}

\endinput


\State{\Struct $\Request$($\timestamp$ : int, $\dot$ : pair$\langle$int, int$\rangle$, \par
         \hskip 4.7em $\strongOp$ : boolean, $\opn$ : $\ops(\FF)$)}

\Operator{$<$}{$r : \Request$, $r' : \Request$}
    \State{\Return $(r.\timestamp, r.\dot) < (r'.\timestamp, r'.\dot)$}
\EndOperator

\State{\Var $\boxx$ : Box}
\State{\Var $\currentEventNumber$ : int}
\State{\Var $\committed$, $\tentative$ : list$\langle\Request\rangle$}
\State{\Var $\executed$, $\toBeExecuted$, $\toBeRolledBack$ : list$\langle\Request\rangle$}
\State{\Var $\requestAwaitingResponse$ : $\Request$}
\State{\Var $\lastResponse$ : $\Response$}

\Upon{$\invoke$}{$\opn$ : $\ops(\FF)$, $\strongOp$ : boolean} \label{alg:bayou:invoke}
    \State{$\currentEventNumber = \currentEventNumber + 1$} \label{alg:bayou:currInc}
    \State{\Var $r = \Request(\currentTime, (i, \currentEventNumber), \strongOp, \opn)$}
    \State{\Rbcast $r$} \label{alg:bayou:rbcast}
    \State{\Tobcast $r$} \label{alg:bayou:tobcast}
    \State{$\requestAwaitingResponse = r$}
\EndUpon

\Upon{$\rbdeliver$}{$r$ : $\Request$} \label{alg:bayou:rbdeliver}
    \If{$r \not\in \committed$}
        \State{\Var $\previous = [ x | x \in \tentative \wedge x < r ]$}
        \State{\Var $\subsequent = [ x | x \in \tentative \wedge r < x ]$}    
        \State{$\tentative = \previous \cdot r \cdot \subsequent$} \label{alg:bayou:rbdeliver_tentative}
        \State{\Var $\newOrder = \committed \cdot \tentative$}
        \State{\Call{$\adjustExecution$}{$\newOrder$}}
    \EndIf
\EndUpon

\Upon{$\tobdeliver$}{$r$ : $\Request$} \label{alg:bayou:tobdeliver}
%      \State{$\newTentative = [ x | x \in \tentative \wedge x \neq r ]$}
    
     \State{$\committed = \committed \cdot r$} \label{alg:bayou:tobdeliver_committed}
%      \State{$\tentative = \newTentative$}
    \State{$\tentative = [ x | x \in \tentative \wedge x \neq r ]$} \label{alg:bayou:tobdeliver_tentative}
\columnbreak    
     \State{\Var $\newOrder = \committed \cdot \tentative$}
     \State{\Call{$\adjustExecution$}{$\newOrder$}}
     
     \If{$r = \requestAwaitingResponse \wedge r \in \executed$}
%          \State{$\response = \lastResponse$}
%          \State{return $\response$ to client}
         \State{return $\lastResponse$ to client}
         \State{$\requestAwaitingResponse = \bot$}
     \EndIf
\EndUpon



\Function{$\adjustExecution$}{$\newOrder$ : list$\langle\Request\rangle$}
    \State{\Var $\inOrder =\ $longestCommonPrefix$(\executed, \newOrder)$}
    \State{\Var $\outOfOrder = [ x | x \in \executed \wedge x \not\in \inOrder ]$}
    
%     \If{$\inOrder \neq []$}
        \State{$\executed = \inOrder$}
        \State{$\toBeExecuted = [ x | x \in \newOrder \wedge x \not\in \executed ]$}
        \State{$\toBeRolledBack = \toBeRolledBack \cdot \reverse(\outOfOrder)$}
%     \EndIf
\EndFunction

\Upon{$\toBeRolledBack \neq []$}{}
    \State{\Var $[ \head ] \cdot \tail = \toBeRolledBack$}
    \State{$\boxx.\rollback(\head)$} \label{alg:bayou:rollback}
    \State{$\toBeRolledBack = \tail$}
\EndUpon
    
\Upon{$\toBeRolledBack = [] \wedge \toBeExecuted \neq []$}{}
    \State{\Var $[ \head ] \cdot \tail = \toBeExecuted$}
    \State{\Var $\response = \boxx.\execute(\head)$} \label{alg:bayou:execute}
    
    \If{$\head = \requestAwaitingResponse$}
        \State{$\lastResponse = \response$}
        \If{$\neg \head.\strongOp \vee \head \in \committed$}
            \State{return $\response$ to client}
            \State{$\requestAwaitingResponse = \bot$}
        \EndIf
    \EndIf
    
    \State{$\executed = \executed \cdot \head$}
    \State{$\toBeExecuted = \tail$}
\EndUpon

\end{algorithmic}
\end{multicols*}
\vspace{-0.4cm}
\end{algorithm*}

\endinput

initialisation:
  received = \emptyset  // was received_p
  unordered = \emptyset // was unordered_p
  ordered = []          // was ordered_p
  k = 0

procedure CA-broadcast(m, p) 
  msg.m = m
  msg.p = p
  R-broadcast message(msg) to all

procedure rcv(ids)
  return \forall id \in ids : exists msg \in received : id(msg) = id \wedge msg.p

when R-deliver message(msg)
  received = received \cup \{ msg \}
  if id(msg) \not\in ordered then
    unordered = unordered \cup \{ id(msg) \}
    
when unordered \neq \emptyset 
  k = k + 1
  propose(k, unordered, rcv) 
  wait until decide(k, idSet_k)
  unordered = unordered \setminus idSet_k
  idSeq_k = elements of idSet_k (in some deterministic order)
  ordered = ordered \cdot idSeq_k

when ordered \neq \emptyset and \exists m \in received : ordered.head = id(m)
  CA-deliver(m)
  ordered = ordered.tail


==> algorithms/creekmv_alg.tex <==
\begin{algorithm*}%[p] 
\caption{The CreekMV protocol for replica $i$}
\label{alg:creekmv}  
% \algsetup{linenosize=\tiny}
  \footnotesize
\vspace{-0.15cm}
\begin{multicols*}{2}
\begin{algorithmic}[1]
\State{\Struct $\VersionId$($\timestamp$ : int, $\dot$ : pair$\langle$int, int$\rangle$)}
\Operator{$<$}{$\vid : \VersionId$, $\vid' : \VersionId$}
    \State{\Return $(\vid.\timestamp, \vid.\dot) < (\vid'.\timestamp, \vid'.\dot)$}
\EndOperator

\State{\Struct $\Request$($\vid$ : $\VersionId$, $\strongOp$ : boolean, $\opn$ : $\ops(\FF)$, \par
         \hskip 4.7em $\causalContext$ : dvv))}

\Operator{$<$}{$r : \Request$, $r' : \Request$}
    \State{\Return $r.\vid < r'.\vid$}
\EndOperator

\State{\Var $\boxx$ : BoxMV}
\State{\Var $\currentEventNumber$ : int}
\State{\Var $\committed$, $\tentative$ : list$\langle\Request\rangle$}
\State{\Var $\causalContext$ : dvv \hfill // logically set$\langle$pair$\langle$int, int$\rangle\rangle$}
\State{\Var $\pendingStrongRequests$ : list$\langle\Request\rangle$}
\State{\Var $\executed$, $\toBeExecutedOrReexecuted$ : list$\langle\Request\rangle$}
\State{\Var $\possibleConflicts$ : map$\langle\Request, $list$\langle\Request\rangle\rangle$}
\State{\Var $\tentativelyExecuted$ : set$\langle\Request\rangle$}
\State{\Var $\unconfirmed$ : set$\langle\Request\rangle$}
\State{\Var $\requestAwaitingResponse$ : $\Request$}
\State{\Var $\lastResponse$ : $\Response$}
% 
\Upon{$\tobcastProposal$}{$r$ : $\Request$}
    \If{$\causalContext \subseteq r.\causalContext$}
        \State{respond to leader $\voteOK(r)$}
    \Else
        \State{$\unconfirmed = \unconfirmed \cup \{ r \}$}
    \EndIf
\EndUpon

\Function{$\checkUnconfirmed()$}{}
    \For{$x \in \unconfirmed$}
        \If{$x.\causalContext \subseteq \causalContext$}
            \State{respond to leader $\voteOK(x)$}
        \EndIf
    \EndFor
\EndFunction

\Upon{$\invoke$}{$\opn$ : $\ops(\FF)$, $\strongOp$ : boolean} \label{alg:creekmv:invoke}
    \State{$\currentEventNumber = \currentEventNumber + 1$} \label{alg:creekmv:currInc}
    \State{\Var $r = \Request(\VersionId(\currentTime, (i, \currentEventNumber)),$ \par
        \hskip 7.5em $\strongOp, \opn)$}
    \If{$\strongOp$}
        \State{$r.\causalContext = \causalContext$}
        \State{\Rbcast $r$ \hfill // optional} \label{alg:creekmv:rbcast}
        \State{\Tobcast $r$} \label{alg:creekmv:tobcast}
    \Else
        \State{\Rbcast $r$}
    \EndIf
    \State{$\requestAwaitingResponse = r$}
\EndUpon

\Upon{$\rbdeliver$}{$r$ : $\Request$} \label{alg:creekmv:rbdeliver}
    \If{$r \not\in \committed$}
        \State{$\causalContext = \causalContext \cup \{ r.dot \}$}
        \State{\Call{$\checkUnconfirmed()$}{}}
        \State{\Call{$\adjustTentativeOrder$}{$r$}}
        \State{\Call{$\checkPendingStrongRequests()$}{}}
    \EndIf
\EndUpon

\Upon{$\tobdeliver$}{$r$ : $\Request$} \label{alg:creekmv:tobdeliver}
     \State{$\pendingStrongRequests = \pendingStrongRequests \cup \{ r \}$} 
     \State{\Call{$\checkPendingStrongRequests()$}{}}
\EndUpon

% \columnbreak   

\Function{$\adjustTentativeOrder$}{$r$ : $\Request$}
     \State{\Var $\previous = [ x | x \in \tentative \wedge x < r ]$}
     \State{\Var $\subsequent = [ x | x \in \tentative \wedge r < x ]$}    
     \State{$\tentative = \previous \cdot r \cdot \subsequent$} \label{alg:creekmv:rbdeliver_tentative}
     \State{\Var $\newOrder = \committed \cdot \tentative$}
     \State{\Call{$\adjustExecution$}{$\newOrder$}}
\EndFunction
% 
\Function{$\adjustExecution$}{$\newOrder$ : list$\langle\Request\rangle$}
    \State{\Var $\inOrder =\ $longestCommonPrefix$(\executed, \newOrder)$}
    \State{$\executed = \inOrder$}
%     \State{$\toBeExecutedOrReexecuted = [ x | x \in \newOrder \wedge x \not\in \executed ]$}
    \State{$\toBeExecutedOrReexecuted = [ x | x \in \newOrder$ \par
        \hskip 13.8em $\wedge\ x \not\in \executed ]$}
\EndFunction

\Function{$\checkPendingStrongRequests$()}{}
    \While{$[ \head ] \cdot \tail = \pendingStrongRequests$ \\ 
    \hskip 4.2em  $\wedge\ \head.\causalContext \subseteq \causalContext$} 
        \State{$\pendingStrongRequests = \tail$}
        \State{$\causalContext = \causalContext \cup \{ r.\dot \}$}
        \State{\Call{$\commit$}{$\head$}}
    \EndWhile
\EndFunction

% \columnbreak
 
\Function{$\commit$}{$r$ : $\Request$}
    \State{$\committedExtension = [ x | x \in \tentative$ \\
       \hskip 12.5em $\wedge\ x.\dot \in r.\causalContext$}
    \State{$\newTentative = [ x | x \in \tentative \wedge x \not\in \committedExtension$ \\
       \hskip 9.5em $\wedge\ x \neq r ]$}
    \State{$\committed = \committed \cdot \committedExtension \cdot r$}
    \State{$\tentative = \newTentative$}
    \State{\Var $\newOrder = \committed \cdot \tentative$}
    \State{\Call{$\adjustExecution$}{$\newOrder$}}
    
    \For{$r' \in \committedExtension \cdot r$}
        \If{$r' \not\in \executed$}
            \State{\Break}
        \EndIf
        \State{$\boxx.\promoteToCommitted(r')$}
        \If{$r' = \requestAwaitingResponse$}
            \State{return $\lastResponse$ to client}
            \State{$\requestAwaitingResponse = \bot$}
        \EndIf
    \EndFor
    
    \For{$r' \in \committedExtension : r' \in \tentativelyExecuted$}
        \For{$r'' \in \newTentative : r'' \in \tentativelyExecuted$}
            \If{$r'' < r'$}
                \State{$\possibleConflicts[r'] = \possibleConflicts[r'] \cup \{ r'' \}$}
            \Else
                \State{$\possibleConflicts[r''] = \possibleConflicts[r''] \cup \{ r' \}$}
            \EndIf
        \EndFor
    \EndFor
    
\EndFunction
% 
% \Upon{$\toBeRolledBack \neq []$}{}
%     \State{$[ \head ] \cdot \tail = \toBeRolledBack$}
%     \State{$\boxx.\rollback(\head)$} \label{alg:creekmv:rollback}
%     \State{$\toBeRolledBack = \tail$}
% \EndUpon

\Upon{$\toBeExecutedOrReexecuted \neq []$}{}
    \State{\Var $[ \head ] \cdot \tail = \toBeExecutedOrReexecuted$}
    
    \State{\Var $\hasBeenAlreadyExecuted = \head \in \tentativelyExecuted$}
    \State{\Var $\rs = \boxx.\readset(\head)$}
    \State{\Var $\rollbackRequired = \false$}
    \If{$\hasBeenAlreadyExecuted \wedge \rs \neq \emptyset$}
        \For{$r' \in \possibleConflicts[\head]$}
            \If{$\boxx.\writeset(r') \cap \rs \neq \emptyset$}
                \State{$\rollbackRequired = \true$}
                \State{\Break}
            \EndIf
        \EndFor
        \If{$\rollbackRequired$}
            \State{$\boxx.\rollback(\head)$}
        \EndIf
    \EndIf
    
    \If{$\neg \hasBeenAlreadyExecuted \vee \rollbackRequired$}
        \State{\Var $\isCommitted = \head \in \committed$}
        \State{\Var $\response = \boxx.\execute(\head, \isCommitted)$} \label{alg:bayoumv:execute}
        \For{$r' \in \tail$}
            \If{$r' \in \tentativelyExecuted$}
                \State{$\possibleConflicts[r'] = \possibleConflicts[r'] \cdot \head$}
            \EndIf
        \EndFor
        \If{$\head = \requestAwaitingResponse$}
            \State{$\lastResponse = \response$}
            \If{$\neg \head.\strongOp \vee \head \in \committed$}
                \State{return $\response$ to client}
                \State{$\requestAwaitingResponse = \bot$}
            \EndIf
        \EndIf
    \EndIf
    \If{$\head \in \committed$}
        \State{$\tentativelyExecuted = \tentativelyExecuted \setminus \{ \head \}$}
    \Else
        \State{$\tentativelyExecuted = \tentativelyExecuted \cup \{ \head \}$}
    \EndIf
    \State{$\executed = \executed \cdot \head$}
    \State{$\toBeExecutedOrReexecuted = \tail$}
\EndUpon

\end{algorithmic}
\end{multicols*}
\vspace{-0.4cm}
\end{algorithm*}

\endinput


==> algorithms/mvdb_alg.tex <==
\begin{algorithm}[t] 
\caption{MvDB for some replica}
\label{alg:box}  
% \algsetup{linenosize=\tiny}
  \footnotesize
% \vspace{-0.15cm}
% \begin{multicols*}{2}
\begin{algorithmic}[1]
\State{\Const $\CommittedVersionId = \VersionId(0, (0, 0))$}
\State{\Struct $\Entry$($v$ : $\Value$, $\vid$ : $\VersionId$)}

\State{\Var $\db$ : map$\langle\Id,\ $list$\langle\Entry\rangle\rangle$}

\Function{$\getTentative$}{$\idd$ : $\Id$, $\vid$ : $\VersionId$}
    \State{\Var $\previous = [ x | x \in \db[\idd] \wedge x.\vid \leq \vid ]$}
    \If{$\front \cdot [ \last ] = \previous$}
        \State{\Return $\last.v$}
    \Else
        \State{\Return $\bot$}
    \EndIf
\EndFunction
 
\Function{$\getCommitted$}{$\idd$ : $\Id$}
    \State{\Return \Call{$\getTentative$}{$\idd, \CommittedVersionId$}}
\EndFunction

\Function{$\insertTentative$}{$\idd$ : $\Id$, $v$ : $\Value$, $\vid$ : $\VersionId$}
    \State{\Var $e = \Entry(v, \vid)$}
%     \State{\Var $\listt = \db[\idd]$}
    \State{$\previous = [ x | x \in \db[\idd] \wedge x.\vid < \vid ]$}
    \State{$\subsequent = [ x | x \in \db[\idd] \wedge x.\vid > \vid ]$}
    \State{$\db[\idd] = \previous \cdot e \cdot \subsequent$}
\EndFunction

\Function{$\insertCommitted$}{$\idd$ : $\Id$, $v$ : $\Value$, $\vid$ : $\VersionId$}
    \State{$\db[\idd] = [ x | x \in \db[\idd] \wedge x.\vid \not\in \{ \CommittedVersionId, \vid \} ]$}
    \State{\Call{$\insertTentative$}{$\idd, v, \CommittedVersionId$}}
\EndFunction

\Function{$\remove$}{$\vid$ : $\VersionId$}
    \For{$(\idd, \listt) \in \db$}
        \State{$\db[\idd] = [ x | x \in list \wedge x.\vid \neq \vid ]$}
    \EndFor
\EndFunction

\end{algorithmic}
% \end{multicols*}
% \vspace{-0.4cm}
\end{algorithm}

\endinput



